EC-DIT: Scaling Diffusion Transformers with Adaptive Expert-Choice Routing

Diffusion transformers have been widely adopted for text-to-image synthesis. While scaling these models up to billions of parameters shows promise, the effectiveness of scaling beyond current sizes remains underexplored and challenging. By explicitly exploiting the computational heterogeneity of image generations, we develop a new family of Mixture-of-Experts (MoE) models (EC-DIT) for diffusion transformers with expert-choice routing. EC-DIT learns to adaptively optimize the compute allocated to understand the input texts and generate the respective image patches, enabling heterogeneous computation aligned with varying text-image complexities. This heterogeneity provides an efficient way of scaling EC-DIT up to 97 billion parameters and achieving significant improvements in training convergence, text-to-image alignment, and overall generation quality over dense models and conventional MoE models. Through extensive ablations, we show that EC-DIT demonstrates superior scalability and adaptive compute allocation by recognizing varying textual importance through end-to-end training. Notably, in text-to-image alignment evaluation, our largest models achieve a state-of-the-art GenEval score of 71.68% and still maintain competitive inference speed with intuitive interpretability.

==> ICLR25_submission/sections/preliminary.tex <==
\section{Preliminaries}\label{sec:preliminary}

\paragraph{Image generation via rectified flow.} 
 DiT processes images as sequences of patches in latent space. An input image is first equally divided into a grid of patches, then flattened and projected into embedding sequences. We denote $\xb\in\RR^{S\times d_x}$ as the image sequence of length $S$ in latent space, with $d_x$ representing the model's hidden dimension. Diffusion models progressively perform time-dependent denoising procedures on the image sequence $\xb$. We adopt the rectified flow approach~\citep{rectifiedflowlipman, rectifiedflowliu}, which follows the formulation $\xb_t=t \xb + (1-t)\epsilon$, where $\xb\sim p_0(\xb)$ is sampled from the original data distribution. 
For any $\xb_t\sim p_t(\xb)$ along the probability path between $p_0$ and Gaussian distribution, $\xb_t$ coincides with a probability flow ordinary differential equation (ODE). 
We also define the velocity field as $d\xb_t=v_\theta(\xb_t, t)dt$, which rectifies the flow toward the direction $(\xb_1-\xb_0)$. We parametrize $v_\theta(\xb_t, t)$ with DiT and optimize the following L2 objective~\citep{rectifiedflowliu, sd3}, \ie,
\begin{equation}\label{eq:diffusion_loss} 
\Lcal\rbr{\theta} = \EE_{t\sim \pi\rbr{t}, \epsilon\sim\Ncal\rbr{0, 1}}\sbr{\|(\xb_1-\xb_0)-v_\theta(\xb_t, t)\|^2},
\end{equation}
where $\pi(\cdot)$ refers to the timestep density during training, for which we select the logit-normal sampling strategy~\citep{lognormal}: $t=\log\frac{u}{1-u}$, with $u\sim\Ncal(\mu_t, \sigma_t)$. The hyperparameters $\mu_t$ and $\sigma_t$ control the frequency for intermediate timesteps being sampled during the training process.





==> ICLR25_submission/tables/training_specs.tex <==
\begin{table*}[!htb]
\centering
\caption{\textbf{Training specifications.} All models are trained on \texttt{v4} and \texttt{v5p} TPUs~\citep{tpu}. We denote the TPU models as \texttt{<TPU\_type>-<c>}, where \texttt{c} refers to the number of TPU cores.}
\label{tab:tpu_config}
\vspace{.3em}
\fontsize{8}{10}\selectfont\setlength{\tabcolsep}{0.5em}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{TPU} & \textbf{Model configs} &  \textbf{Input shape} & \textbf{Outer batch} & \textbf{Num groups} & \textbf{Group size} & \textbf{Capacity} \\
\midrule
\texttt{v4-256}     & \method-XL-8E     & 4096, 128 & 16  & 32  & 1024 & 256 \\
\texttt{v4-256}     & \method-XL-16E           &  4096, 128         & 8   & 64  & 1024 & 128 \\
\texttt{v4-256}     & \method-XL-32E           &  4096, 128         & 4   & 128 & 1024 & 64  \\\hline
\texttt{v4-512}     & \method-XXL-8E    & 4096, 128 & 32  & 16  & 1024 & 256 \\
\texttt{v4-512}     & \method-XXL-16E          &  4096, 128         & 16  & 32  & 1024 & 128 \\
\texttt{v5p-512}    & \method-XXL-32E          &  4096, 128         & 8   & 64  & 1024 & 64  \\\hline
\texttt{v5p-512}    & \method-3XL-8E    & 4096, 128 & 32  & 16  & 1024 & 256 \\
\texttt{v5p-512}    & \method-3XL-16E          &  4096, 128         & 16  & 32  & 1024 & 128 \\
\texttt{v5p-512}    & \method-3XL-32E          &  4096, 128         & 8   & 64  & 1024 & 64  \\\hline
\texttt{v5p-1024}   & \method-M-64      & 4096, 128 & 8   & 64  & 1024 & 32  \\
\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table*}
